Integrating Large Circular Kernels into CNNs through Neural Architecture Search

The square kernel is a standard unit for contemporary CNNs, as it fits well on the tensor computation for convolution operation. However, the retinal ganglion cells in the biological visual system have approximately concentric receptive fields. Motivated by this observation, we propose to use circular kernel with a concentric and isotropic receptive field as an option for the convolution operation. We first propose a simple yet efficient implementation of the convolution using circular kernels, and empirically show the significant advantages of large circular kernels over the counterpart square kernels. We then expand the operation space of several typical Neural Architecture Search (NAS) methods with the convolutions of large circular kernels. The searched new neural architectures do contain large circular kernels and outperform the original searched models considerably. Our additional analysis also reveals that large circular kernels could help the model to be more robust to the rotated or sheared images due to their better rotation invariance. Our work shows the potential of designing new convolutional kernels for CNNs, bringing up the prospect of expanding the search space of NAS with new variants of convolutions.

==> Circular Kernel/01Intro.tex <==
The square convolution kernel has been regarded as the standard and core unit of Convolutional Neural Networks (CNNs) since the first recognized CNN of \textit{LeNet}  proposed in 1989~\citep{lecun1998gradient}, and especially after \textit{AlexNet}~\citep{krizhevsky2012imagenet} won the ILSVRC (ImageNet Large Scale Visual Recognition Competition) in 2012. Since then, various variants of convolution kernels have been proposed, including  separable convolution~\citep{chollet2017xception}, dilated convolution~\citep{yu2015multi}, deformable convolution~\citep{jeon2017active,dai2017deformable,zhu2019deformable,gao2019deformable}, \etc. 
Inspired by the fact that the retinal ganglion cells in the biological visual system have approximately concentric receptive fields (RFs)~\citep{hubel1962receptive,simoncelli2001natural,mutch2008object}, we propose the concept of circular kernels for the convolution operation\footnote{Code: https://github.com/JHL-HUST/CircularKernel.}. As shown in Fig. \ref{fig:3-5-7}, a $K \times K$ circular kernel is defined as a kernel that evenly samples $K^2$ pixels on the concentric circles to form a circular receptive field. 

Besides the similarity to biological RFs, we observe that the circular kernel provides many advantages over the square kernel. 
%whose receptive field is formed by
%and with the largest diameter of $K$
%First, the RFs and stacked RFs of circular kernels are more round and similar to the biological RFs.
First, the receptive field of a kernel is traditionally expected to be isotropic to fit thousands of uncertain symmetric orientations of the input feature maps, either globally or locally. An \textit{isotropic} kernel means the kernel samples evenly in different directions of the RFs. The circular kernel is roughly isotropic and rotation-invariant, whereas a square kernel is symmetric only in a few orientations. 
Second, Luo \etal~\citep{luo2017understanding} indicate that the effective RF of a square kernel has a Gaussian distribution which is in a nearly circular shape. It indicates that the meaningful weights are sparse at the four corners of large square kernels or stacked $3 \times 3$ square kernels. Compared to pruning these diluted parameters during the fine-tuning stage~\citep{han2015learning}, directly constructing kernels with the same shape of effective RFs is probably more effective.
\par
 
\input{Figure/3-5-7}
 
%One of the cornerstones
One cornerstone 
of the rationality of employing circular kernels is the isotropic property of circles. However, a $3 \times 3$ circular kernel is not really in circular shape as it only samples nine pixels with a similar arrangement to the square kernel. If we build the circular kernels in larger kernel size, as illustrated in Fig. \ref{fig:3-5-7}, we can see that a larger circular kernel has a more round receptive field and is more distinct from the corresponding square kernel. Our follow-up experiments also demonstrate that the circular kernels exhibit significant advantages over the square kernels on larger kernel sizes.
% in which the receptive field of circular kernels is more round and the difference between circular kernels and square kernels is more obvious. /HK{repetitive sentences}
 
 
The $3 \times 3$ square kernels have become the mainstream of the CNN units since the work of VGG~\citep{simonyan2014very} suggests that a larger square kernel could be substituted by several $3 \times 3$ square kernels utilizing fewer parameters. In recent years, however, the functions of larger square kernels have been considered underestimated, as almost all the powerful models generated by Neural Architecture Search (NAS)~\citep{zoph2018learning,liu2018progressive,DBLP:conf/iclr/XuX0CQ0X20,nayman2019xnas} contain large square kernels, and many manually designed neural architectures also contain large square kernels~\citep{he2016deep,peng2017large,li2019selective}. The recent 
%ConvNeXt~\citep{liu2022convnet} outperforming Swin transformer~\citep{liu2021swin} 
success of ConvNeXt~\citep{liu2022convnet} over Swin transformer~\citep{liu2021swin} 
also shows that 
increasing the kernel size can significantly improve the performance. Compared to small kernels, large kernels have received insufficient attention despite their vast range of applications. 
Hence, we introduce convolutions with large circular kernels 
as an option for the CNN units, especially for NAS. % to serve as excellent candidates for the search space of existing NAS methods.  
\input{Figure/main_fig}

The mainstream CNNs are manually developed and optimized on the $3 \times 3$ square kernels. 
%, which is evident yet often overlooked. 
So variants of kernels encounter significant resistance to outperform $3 \times 3$ square kernels on the existing popular architectures. NAS aims to design a neural architecture that performs best under limited computing resources in an automated manner~\citep{ren2020comprehensive}. It creates a level playing field for different types of operations in the search space. In manually designed architectures, the network typically contains the same unit for all layers (e.g., $3 \times 3$ square kernels) because %we do not know how to 
it is hard to 
arrange them in different layers appropriately if we have several different units. For the convolution operation, although it is hard to substitute the standard convolution with the variants in all layers of the typical manual architectures, NAS enables the variants to exist in the proper position as a part of the overall network. Then some special variants are likely to outperform the standard operations if being located in the right position. Consequently, although existing NAS methods have achieved superior performance, 
their search space that only contains popular operations used in manual architectures seems conservative.

%\HK{This paragraph could be removed. A discussion could be in experiments, but not in intro.}
%A natural idea of improving the operation space of NAS is to expand the space with deformable convolutions~\citep{jeon2017active,dai2017deformable,zhu2019deformable, Gao2020Deformable}, as deformable convolutions work well in manual architectures but are never considered in existing NAS methods. However, because NAS is a complicated bilevel optimization problem even on the standard convolutions~\citep{DBLP:conf/iclr/LiuSY19}, convolutional adaptation methods that require additional parameters are unlikely to be 
%%currently not 
%applicable to NAS due to the excessive optimization and considerable computation overhead.  \par
%%So the ideal operation should preferably not require additional optimization. \par



In this work, we propose to use the convolution of large circular kernels with a concentric and isotropic receptive field as an option for the search space of NAS methods.
As shown in Fig.~\ref{fig:cifar},
%Our preliminary experiments show that 
by simply substituting the $3\times3$ square kernels with $3\times3$ circular kernels in manual CNN architectures, the performance of the modified network after training could be on par with the original network, even though the original one is designed and hence optimized manually on square kernels.
Moreover, with the increment of kernel size on the modified models adapted on typical manual models, although the overall performance declines for both square kernels and circular kernels, the circular kernels actually exhibit significantly increasing advantages over the counterpart square kernels. 
%  the increasing advantages of circular kernels over the square kernels 
%as the kernel size increases and the difference is more distinct, 
%with the increment of the kernel size, 
%and the difference of the two types of kernels is more distinct. 
%although the overall performance decreases with the kernel size increases. 
%We notice that these typical CNN architectures are manually designed and optimized based on the square kernels that are usually in size $3 \times 3$. %CNN with convolutions that completely composed of large kernels is not superior and more time consuming. 

Our preliminary experiments inspire us to expand the search space of NAS methods with convolutions of large circular kernels. In this way, NAS %probably 
may enable the convolutions of large circular kernels to be located in \textbf{proper position} to outperform the standard operations. 
Note that many works have shown that simply enlarging the operation space could be detrimental to the final results~\citep{DBLP:conf/iclr/YuSJMS20,DBLP:journals/pami/ZhangHWXP21,ci2020evolving}. 
%So although we expand the operation space with convolutions of the large circular kernels, the performance will not be simply improved if large circular kernels are useless.
Hence, our method of expanding the operation space with convolutions of large circular kernels is beneficial for the NAS. 



Our main contributions are as follows:
\begin{itemize}[leftmargin=20pt]
	\vspace{-1.5mm}
	\item We first propose to use the circular kernel with a concentric and isotropic receptive field as an option for the convolution operation, especially for the convolution of kernels with larger kernel size.
	 %for improving training efficiency and reducing memory cost of the super-net during search. 
	%\vspace{-1.5mm}
	\item We propose a simple yet efficient implementation for the convolution of the circular kernel, enabling it to work together seamlessly with any CNNs with %negligible 
	little extra time. We also show that the circular kernel has an optimization path different from that of the square kernel.
	%\vspace{-1.5mm}
	\item We propose to use the convolution of large circular kernels as an option for the search space of NAS methods because they enable large circular kernels to be located in proper position, and our experiments show that the searched architectures contain large circular kernels and outperform the original ones containing only square kernels. %CIFAR-10 and ImageNet datasets.  on three datasets
	%\vspace{-1.5mm}
	\item Our study reveals an important phenomenon that the variants, that perform averagely in manual architecture because of inherent mode of thinking, probably have extraordinary performance in neural architecture search. We emphasize that the search space can be expanded as new designs emerge.
	%\item Experimental results of NAS show that the searched architectures contain large circular kernels and outperform the original ones containing only square kernels for both CIFAR-10 and ImageNet datasets. Further experiments reveal that the large circular kernel help the model to be more robust to rotated or sheared images due to its better rotation invariance.
	%\vspace{-1.5mm}
	%\item We brought up the prospect 
	%Our work shows the potential of designing other shapes of convolutional kernels for CNNs, and especially bringing up the prospect of expanding the search space of NAS with new variants of convolutions.
	%expanding the search space of NAS with convolutions using new variants of kernels.%, and may inspire more work in this direction.
	%variants of convolutions %that don't work as a whole in manual architecture but work as a part in the proper position.
\end{itemize}








==> Circular Kernel/02RW.tex <==
Understanding and exploring the convolution units has always been an essential topic in the field of deep learning. 
In this section, we review the previous primary efforts on the design of convolution kernel and CNN architecture, then show how our work differs.    
\vspace{1ex}

\textbf{Convolution Kernel Design.}
The grouped convolution uses a group of convolutions (multiple kernels per layer) to allow the network to train over multi-GPUs~\citep{krizhevsky2012imagenet}.
The depthwise separable convolution decomposes a standard convolution into a depthwise convolution followed by a pointwise convolution~\citep{chollet2017xception}. 
The spatially separable convolution decomposes a $K \times K$ square kernel into two separate units, a $K \times 1$ kernel and a $1 \times K$ kernel~\citep{mamalet2012simplifying}.
The dilated convolution is a type of convolution that “inflate” the kernel by inserting holes between the kernel elements~\citep{yu2015multi}. 
All the above variants consider large kernels but inherit the square kernel in general.
\vspace{1ex}

In contrast, the deformable convolution~\citep{dai2017deformable,zhu2019deformable} allows the shape of the receptive field to be learnable based on the input feature maps to provide flexibility, but it needs to take considerable extra parameters and computation overhead. Similarly, the deformable kernel~\citep{gao2019deformable} resamples the original kernel space while keeping the receptive field unchanged. There are also many interesting variants with special shapes, including quasi-hexagonal convolution~\citep{sun2016design}, blind-spot convolution~\citep{krull2019noise2void}, asymmetric convolution~\citep{ding2019acnet}, \etc. The above variants change the kernel shape but ignore large kernels. 


In the early stage of CNN design, the kernel size gradually evolves from large to small. In AlexNet, large kernels (e.g., $11\times 11$, $5\times 5$) are used together with $3 \times 3$ kernels. Subsequently, VGG~\citep{simonyan2014very} suggests that a large kernel could be substituted by several $3 \times 3$ kernels utilizing fewer parameters. Then, the smallest $1 \times 1$ kernels are proposed for dimension reduction and efficient low dimensional embedding~\citep{szegedy2015going}. Recently, due to the emergence of NAS, large kernels (e.g., $5\times 5$, $7\times 7$) %have been back to human's sight
have been reemerged and attracted the researchers' attention, 
and become one of the standard units for the searched CNNs. ProxylessNAS~\citep{cai2018proxylessnas} argues that large kernels are beneficial for CNNs to preserve more information for the downsampling. 

\textbf{CNN Architecture Design.} 
Since AlexNet achieved fundamental progress in the ILSVRC-2012 image classification competition~\citep{krizhevsky2012imagenet}, a number of outstanding manual CNN structures emerged, including VGG~\citep{simonyan2014very}, Inception~\citep{szegedy2015going}, ResNet~\citep{he2016deep}, DenseNet~\citep{huang2017densely}, \etc. However, designing the neural architecture heavily relies on researchers’ prior knowledge, but existing prior knowledge and inherent mode of thinking  
are likely to limit the discovery of new neural architectures to a certain extent. As a result, neural architecture search (NAS) was developed to search good CNN structures automatically.


%NAS has brought up the prospect of automating the customization of deep neural architecture for specific applications.
NAS-RL~\citep{DBLP:conf/iclr/ZophL17} and MetaQNN~\citep{DBLP:conf/iclr/BakerGNR17} using reinforcement learning (RL) are considered pioneers in the field of NAS. 
%Follow-up studies focus on reducing the time cost~\citep{Zhong_2018_CVPR,pmlr-v80-cai18a,pham2018efficient}. 
Subsequently, evolution-based algorithms use an evolving process towards better performance to search for novel neural architectures~\citep{xie2017genetic,real2017large,liu2017hierarchical,elsken2018efficient}. To address the issue of high computational demand and time cost in the search scenario, the one-shot method constructs a super-net~\citep{brock2017smash,bender2018understanding}, which is trained once in search and then deemed as a performance estimator. Some studies sample a single path~\citep{guo2019single,li2019random,you2020greedynas} in a chain-based search space~\citep{hu2020dsnas,cai2019once,mei2019atomnas,yu2020bignas} to train the super-net. Another line of gradient-based methods~\citep{DBLP:conf/iclr/LiuSY19,chen2019progressive,chu2020fair,DBLP:conf/iclr/XuX0CQ0X20,DBLP:conf/icml/ChenH20,yang2021towards,DBLP:conf/iclr/ChuW0LWY21} employs the gradient optimization method to perform differentiable joint optimization between the architecture parameters and the super-net weights in a cell-based space efficiently. Some gradient-based methods have reduced the search time significantly to about $0.1$ GPU-days~\citep{DBLP:conf/iclr/XuX0CQ0X20,yang2021towards}.


The search space of all the above works contains convolutions with large kernels that extensively exist in the final searched architectures. However, all the large kernels in these works directly inherit the square shape of the standard $3 \times 3$ kernel. Moreover, all the above works only employ operations that are popular in manual architectures to their operation space. Our work proposes to use convolutions of large circular kernels, which are more distinctive to the counterpart square kernels, to enrich the operation space for automatic neural architecture search. In turn, NAS may enable the convolutions of large circular kernels to be located in proper position to outperform the standard operations.
As far as we know, this work is the first that involves the unpopular variants in the search space of NAS. 




==> Circular Kernel/03Method.tex <==
\input{Figure/square-circle}
This section introduces the circular kernel that evenly samples pixels on concentric circles to form circular receptive fields. We adopt bilinear interpolation for the approximation and re-parameterize the weight matrix by the corresponding transformation matrix to replace the receptive field offsets, thus the training takes an approximately equivalent amount of calculation compared to the standard square convolution. 
We then provide preliminary analysis on %the effect of 
the transformation matrix during training.
In the end, we show how to incorporate large circular kernels into the NAS methods.



\subsection{Circular Kernel versus Square Kernel} 
Without loss of generality, we take the $3 \times 3$ kernel as an example. 
The receptive field $\sS$ of a $3 \times 3$ standard square kernel with dilation 1, 
as shown in Fig. \ref{fig:square-circle} (a),
can be presented as: 
\begin{equation} 
%\resizebox{.9\hsize}{!}{
\begin{aligned}
\sS=&\{(-1,\ \ 1 ),(0,\ \ 1 ),(1,\ \ 1 ),(-1,\ \ 0 ),(0,\ \ 0 ), \\
     &(1,\ \ 0 ),(-1, -1),(0,\  -1),(1,\  -1)\},
\end{aligned} %}
\end{equation}
where $\sS$ denotes the set of offsets in the neighborhood considering the convolution conducted on the center
pixel. By convolving an input feature map $\mI \in \real^{H \times W}$ with a kernel $\mW \in \real^{K \times K}$ of stride 1, we have an output feature map $\mO \in \real^{H \times W}$,
 %commonly used for neural networks,
whose value at each coordinate $\vj$ is:
\begin{equation}
    \label{eq.standard_conv}
	\mO_{j} = \sum_{s \in \sS} \mW_{s} \mI_{j + s}.
\end{equation}
So we have $\mO = \mathbf{W} \otimes \mI$ where $\otimes$ indicates a typical 2D convolution operation used in CNNs.% and $RF(j)$ indicates the receptive field centered on the location $j$.
% Hadamard product / element-wise product of two matrices $\odot



In contrast, the receptive field of a $3 \times 3$ circular kernel can be presented as: 
%\begin{small}
\begin{equation}
\begin{aligned}
\sR=&\{(-\tfrac{\sqrt{2}}{2},\tfrac{\sqrt{2}}{2}),(0,\ \ 1),(\tfrac{\sqrt{2}}{2}, \tfrac{\sqrt{2}}{2}),
               (-1,\  0 ),
               (0,\ 0 ),\\ 
               &(1,\ \ 0),
               (-\tfrac{\sqrt{2}}{2}, -\tfrac{\sqrt{2}}{2}), (0, \ -1),(\tfrac{\sqrt{2}}{2},-\tfrac{\sqrt{2}}{2})\}.
\end{aligned}
%\end{split}
\end{equation}
%\end{small}
As shown in Fig. \ref{fig:square-circle} (b), we resample the input $\mI$ with a group of offsets to each discrete kernel position $\bm{s}$, denoted as $\{\Delta\vr\}$, to form the circular receptive field. The corresponding convolution becomes:
\begin{equation}
    %\label{eq.defor_conv}
    \mO_{j} =  \sum_{\bm{s}\in \sS} \mW_{\bm{s}} \mI_{\vj+\bm{s}+\Delta\vr}.
\label{eq.circle_conv}
\end{equation}
In other words, the value of each entry is the sum of the element-wise products of the kernel weights and the corresponding pixel values in the circular receptive field. 
As the sampling positions of a circular kernel contains fractional positions, we employ bilinear interpolation to approximate the corresponding sampling values inside the circular receptive field: 
% \begin{equation}
% \mI_{\vj+\bm{s}+\Delta\vr}=\sum_{\bm{s} \in \sS} \mathcal{B}(\vj+\bm{s},\vj+\bm{s}+\Delta\vr) \mI_{\vj+\bm{s}},
% \label{eq.bilinear_interpolation_x}
% \end{equation}
\begin{equation}
\mI_{\vr}=\sum_{\bm{s} \in \sS} \mathcal{B}(\bm{s},\vr) \mI_{\bm{s}},
\label{eq.bilinear_interpolation_x}
\end{equation}
where $\vr$ denotes a grid or fractional location in the circular receptive field, $\bm{s}$ enumerates all 
%integral spatial
the grid locations in the corresponding square receptive filed, and $\mathcal{B}(\cdot,\cdot)$ is a two dimensional bilinear interpolation kernel. $\mathcal{B}$ can be separated into two one-dimensional kernels as $\mathcal{B}(\bm{s},\vr)=g(\bm{s}_x,\vr_x)\cdot g(\bm{s}_y,\vr_y)$, where $g(a,b)=max(0,1-|a-b|)$. 
So $\mathcal{B}(\bm{s},\vr)$ 
is non-zero and in (0,1) 
only for the nearest four grids $\bm{s}$ in $\sS$ around fractional location $\vr$, and $\mathcal{B}(\bm{s},\vr) = 1$ only for the corresponding grid $\bm{s}$ in $\sS$ for grid location $\vr$. 






\subsection{Re-parameterization of the Weights}
\label{Re-parameterization}
%In Section~\ref{sec.learnable_kernels}, we use the transformation matrix of bilinear interpretation with values inside the standard square receptive field to simplify the calculation. 
%calculate the offsets for each convolution when the kernel scans the input feature map step by step
Implementing the convolution of a circular kernel that can operate efficiently is not trivial. Considering when building the convolution of a circular kernel, as the offsets of the sampling points in a circular receptive field relative to a square receptive field are fixed, we extract the transformation matrix $\mB$ of the whole receptive field by arranging $\mathcal{B}$ of one pixel $\vr$ in \Eqref{eq.bilinear_interpolation_x}. 

Let $\hat{\mI}_{RF(\vj)} \in \real^{K^2 \times 1}$ and $\hat{\mW} \in \real^{K^2 \times 1}$ represent the resized receptive field centered on the location $j$ and the kernel, respectively. The standard convolution can be defined as $\mO_{j}=\hat{\mW}^{\top}\hat{\mI}_{RF(\vj)}$. 
Then the convolution of circular kernel can be defined as:  
\begin{equation}
\mO_{j}=\hat{\mW}^{\top}\left(\mB\hat{\mI}_{RF(\vj)}\right) = \left(\hat{\mW}^{\top}\mB\right)\hat{\mI}_{RF(\vj)},
\label{eq.conv}
\end{equation}
where $\mB\in \real^{K^2 \times K^2}$ is a fixed sparse coefficient matrix. 
%As the transformation matrix $\mB$ is a fixed coefficient matrix, ~\Eqref{eq.conv} satisfies the associative law of multiplication.
Correspondingly, let $\mI \in \real^{H \times W}$, $\mO \in \real^{H \times W}$ and $\mW \in \real^{K \times K}$ respectively represent the input feature map,  output feature map and the kernel, % and transformation matrix of the bilinear interpolation for a kernel. 
%We have $\mW \otimes \mI$ to represent the convolution of feature map $\mI$ and square kernel $\mW$. 
the convolution of a circular kernel could be briefly defined as:
\begin{equation}
\mO=\mW \otimes \left(\mB\star\mI\right)=\left(\mW \star \mB \right)\otimes\mI, 
\label{eq.trans}
\end{equation}
where $\mB\star\mI$ %represents
is to change the square receptive field to circular receptive field.

%$\mO_{j}=\left(\mW \star \mB\right)\otimes\mI_{RF(j)}$.
%Then, an operation on the original kernel $\mW$ can replace the receptive field offsets.
In this way, we could apply an operation on the kernel weights once to have $\mW \star \mB $ before the kernel scans the input feature map.
Consequently, we do not need to calculate the offsets for each convolution as deformable methods do when the kernel scans the input feature map step by step
~\citep{jeon2017active,dai2017deformable,zhu2019deformable,gao2019deformable}. 
While calculating the receptive field offsets for each convolution is very time-consuming, the computational cost of operations on kernels is negligible compared to the gradient descent optimization. %Thus the training of the convolutions of circular kernel takes an approximately equivalent amount of calculation compared to the standard square convolution.


\subsection{Analysis on Transformation Matrix}
\label{transformation}
%This subsection provides a theoretical analysis of the actual effect of the transformation matrix. %For simplicity, we omit the subscripts related to positions throughout this subsection.
This subsection briefly concludes the analysis of the actual effect of the transformation matrix. 
For a circular kernel, let $\Delta \mW = \mW^{t+1}-\mW^t$. The squared value of a change on the output $\Delta \mO = \mO^{t+1}-\mO^t$ can be calculated as 
$\| \Delta \mO \|^2 = \left( \mB\star \mI \right)^{\top} \otimes \Delta \mW^{\top} \Delta \mW \otimes \left( \mB\star \mI \right)$, which can be transferred to
$\| \Delta \mO \|^2 = \mI^{\top} \otimes \left( \mB^{\top}\star \Delta\mW^{\top} \Delta \mW \star \mB  \right) \otimes\mI$. 
In contrast, $\Delta \widetilde\mO$ of the traditional convolutional layers is determined by $\Delta \mW^{\top} \Delta \mW$ and $\mI$. 
Hence, we can conclude that the transformation matrix $\mB$ affects the %optimal
optimization paths of gradient descent. 
For detailed analysis, see the Supplementary. 
% $A$. %\ref{appendix:transformation}. 
We also empirically demonstrate this claim in Section~\ref{sec:3x3-Kernel}.


%\input{Table/large-circular-kernel}


%\subsection{Neural Architecture Search with Large Circular Kernels}
\subsection{NAS with Large Circular Kernels}
Theoretically, we could expand the operation space of any NAS method with large circular kernels. 
As the one-shot methods yield significant advantage in the time cost over the reinforcement learning or evolutionary-based NAS methods, and the typical one-shot methods of gradient-based ones~\citep{DBLP:conf/iclr/LiuSY19,chen2019progressive,DBLP:conf/iclr/XuX0CQ0X20,yang2021towards} enable us to discover more complex connecting patterns, we adopt them as the baselines for incorporating the large circular kernels.
%existing NAS approaches contain three main categories according to the heuristics to explore the architecture space: reinforcement learning, evolutionary algorithm, and gradient optimization. 
%NASNet~\citep{zoph2018learning}, AmoebaNet~\citep{real2019regularized} are separately considered as the most representative networks of reinforcement learning and evolutionary algorithm. However, NASNet spends 2000 GPU-days to obtain the best architecture in CIFAR-10. Similarly, AmoebaNet spends 3150 GPU-days. 
%Due to the limited time, we search the operation space containing large circular kernels using fast gradient optimization methods.\par

The search space for typical gradient-based methods is made up of cell-based microstructure repeats. Each cell can be viewed as a directed acyclic graph with $N$ nodes and $E$ edges, where each node $x^i$ represents a latent representation (\eg, a feature map), and each edge is associated with operations $o(\cdot)$ (\eg, {\it identity connection}, {\it sep\_conv\_3x3}) in the operation space $\mathcal{O}$. Within a cell, the goal is to choose one operation from $\mathcal{O}$ to connect each pair of nodes. %Note that simply enlarging the search space could be detrimental to the final according to ~\citep{DBLP:conf/iclr/YuSJMS20,DBLP:journals/pami/ZhangHWXP21,ci2020evolving}. 
% for the NAS methods. 

Let a pair of nodes be $\left(i,j\right)$, where ${1}\leqslant{i}<{j}\leqslant{N}$, the core idea of typical gradient-based methods is to formulate the information propagated from $i$ to $j$ as a weighted sum over $\left|\mathcal{O}\right|$ operations as the mixed operation: %following equation:
\begin{small}
\begin{align}
	\bar{o}^{(i,j)}\left(w,\mathbf{x}_i\right) = \sum_{o \in \mathcal{O}} \frac{\exp(\alpha_o^{(i,j)})}{\sum_{o' \in \mathcal{O}} \exp(\alpha_{o'}^{(i,j)})} o\left(w_o^{(i,j)},\mathbf{x}_i\right),
	\label{eq:soft}
\end{align}
\end{small}
where $\mathbf{x}_i$ is the output of the $i$-th node, $\alpha_o^{(i,j)}$ is a hyper-parameter for weighting operation $o\!\left(\mathbf{x}_i\right)$, and $w_o^{(i,j)}$ is the weight. The entire framework is then differentiable to both layer weights in operation $o(\cdot)$ and hyper-parameters $\alpha_o^{(i,j)}$ in an end-to-end fashion.  
After that, a discrete architecture can be obtained by replacing mixed operations with most likely operations at the end of the search. 

The operation space $\mathcal{O}$ of typical gradient-based methods is: $3 \times 3$ and $5 \times 5$ separable convolutions, $3 \times 3$ and $5 \times 5$ dilated separable convolutions, $3 \times 3$ max pooling, $3 \times 3$ average pooling, identity, and \textit{zero}, which only considers convolutions or pooling that are popular in manually designed CNNs. 
Considering variants of convolutions may outperform the popular convolutions when they are located in the proper position, we add $5 \times 5$ circular separable convolutions and $5 \times 5$ circular dilated separable convolutions to the operation space, which are constructed by replacing the square kernels of the separable or dilated convolution with circular kernels.
%More details for the search process can be found in DARTS~\citep{DBLP:conf/iclr/LiuSY19}. 



%, and term the searched architectures as DARTS-Circle and PC-DARTS-Circle.
%This design makes the entire framework differentiable to both layer weights and hyper-parameters $\alpha_{i,j}^o$, so that it is possible to perform architecture search in an end-to-end fashion. 



%Concretely, every operation on an edge is activated during the search phase, with their outputs mixed by the architecture parameter $\alpha$ to form the final mixed output of that edge $\bar{m}(x^i) = \sum_{o\in\mathcal{O}} \frac{\exp \alpha_o}{\sum_{o'} \exp \alpha_{o'}} o(x^i)$. The intermediate node takes the summation of the outputs from all edges from the previous nodes as its value: $\textbf{x}^i = \sum_{j < i} \bar{o}(\textbf{x}^j)$.





% \begin{figure*}[tb]
%     \centering
%     \includegraphics[width=1\textwidth]{parameters_adjustment.pdf}
%     \bm{s}pace{-15pt}
%     \caption{Training the integrated kernels in the overall model. The adaptive parameters $\hbt=\{\hbt_1, \hbt_2,...,\hbt_N\}$ are picked randomly to train together with the essential weights $\bt$ during the iterations.}
%     \bm{s}pace{-10pt}
%     \label{parameters_adjustment}
% \end{figure*}



% \subsection{Training a Model with Integrated Kernels}
% \label{sec.integrate}
% For an input sample $\rvx$, the output of a conventional neural network can be written as: 
% \begin{equation}
% \rvy\! =\! \mathcal{F}(\rvx,\bt).
%   \label{eq:normal_output}
% \end{equation}
% Then, the output of a model with adaptive parameters can be written as $\rvy = \mF(\rvx,\bt, \hbt)$, where $\bt$ represents the basic parameters like weights, and $\hbt$ represents adaptive parameters. \par




% During the training, as illustrated in Figure \ref{parameters_adjustment}, the output of a model with integrated kernels is: 
% \begin{equation}
%   \mathbf{y} = \mathcal{F}(\rvx,\bt, \mathbf{Mul} (\hat{\bt}^l;L,p)),
%   \label{eq:dynamic_parameter}
% \end{equation}
% where $L$ is the number of layers of the CNN model, $\hbt^l=\{\hbt^l_1,...,\hbt^l_n,...,\hbt^l_N\}$ denotes the $N$ sets of parameters related to the kernel shape (square or circle) or size/radius ($a$) in each layer $l$, $p=\{p_1, ..., p_n, ... p_N\}$,
% $\mathbf{Mul}(\hat{\bt}^l;L,p)$ represents that the model selects $\hbt^l_n$ with probability $p_n$ at each layer $l$ for all layers. 
% If we let each $p_n = \tfrac{1}{N}$, the overall model can be regarded as an ensemble of $N^L$ sub-networks during the training phase. 
% In our experiments, $N$ is usually set to 2 and a larger $N$ is discussed in the ablation study of Section~\ref{sec:ablation}. 







==> Circular Kernel/04ExpNew.tex <==
 %\subsection{Experimental Setup}
 %\label{sec:experiment-setup} 
%We empirically demonstrate the effectiveness of circular kernels on the image classification task using standard datasets. We first compare the $3 \times 3$ circular kernels and an integrated version of kernels with the $3 \times 3$ square kernels on ImageNet using manually designed typical neural architectures, ResNet~\citep{he2016deep}. 



In this section, we empirically demonstrate the advantages of large circular kernels 
%compared to 
over large square kernels. 
% by preliminary experiments on CIFAR-10 and CIFAR-100. 
Then we expand the search space of NAS with large circular kernels and apply the strategy described in several representative gradient-based NAS methods to search for new neural network architectures based on their ability of locating large circular kernels in proper position. Experimental results show that the searched architectures contain large circular kernels and outperform the original ones 
on both CIFAR-10 and ImageNet datasets. Detailed experimental setup can be found in the Supplementary. % file.
%An analysis on the robustness of circular kernels is provided in the end. %searched models with



\subsection{The Advantages of Large Circular Kernels}
\label{sec:cifar}
We have shown in Fig.~\ref{fig:3-5-7} that a large circular kernel has a more round receptive field and is more distinguishable from the corresponding square kernel. We conjecture that the larger circular kernels would exhibit a more significant advantage over the square kernels if the circular kernels are helpful for deep learning tasks. To verify this hypothesis, we augment VGG~\citep{simonyan2014very}, ResNet~\citep{he2016deep}, WRNCifar~\citep{zagoruyko2016wide}, DenseNetCifar~\citep{huang2017densely}, and their circular kernel versions with larger kernel sizes and compare their performance on CIFAR-10 and CIFAR-100. For a fair comparison, we show the results of the original data without data augmentation. Results on CIFAR-10 and CIFAR-100 with standard data augmentation can be found in the Supplementary. We run the model 5 times for each dataset \& model setting to reduce the variance.  %$B.1$. %~\ref{sec:CIFAR-10-Artificially}.

As shown in Fig.~\ref{fig:cifar}, 
the performance of both the baselines and the corresponding circular kernel versions basically declines with the increment of the kernel size. Nevertheless, we see that the advantage of circular kernels over square kernels becomes more distinct for larger kernels. The average gain brought by circular kernels on four models is $1.1\%$ for kernel size of $3$, $2.0\%$ for kernel size of $5$, and $2.8\%$ for kernel size of $7$, indicating the superiority of large circular kernels. \par 





% \subsection{Comparison of large Kernels on CIFAR-10 and ImageNet }
% \label{sec:large-Kernel}
% $3 \times 3$ circular kernels are not superior in performance compared to square kernels and take approximately $2\%$ more FLOPs. Consequently, we explore larger kernels in this section. We compare our large circle versions with NASNet~\citep{zoph2018learning}, AmoebaNet~\citep{real2019regularized}, which are separately considered as the most representative networks of reinforcement learning and evolutionary algorithm~\citep{DBLP:conf/iclr/LiuSY19,DBLP:journals/csur/RenXCHLCW21}. However, NASNet spends 2000 GPU-days to obtain the best architecture in CIFAR-10. Similarly, AmoebaNet spends 3150 GPU-days. Due to limited time, we simply replace the large kernels in their searched architectures with circular kernels. 


% \input{Table/NAS-imagenet}


\subsection{Searched Models with Large Circular Kernels}% on CIFAR-10 and ImageNet}
\label{sec:NAS-search}
%In Section \ref{sec:cifar} and \ref{sec:3x3-Kernel}, 
%In the above discussion, the models and hyper-parameters are built by manual design on square kernels. Therefore, it is possible to achieve more remarkable improvement if large circular kernels are added to the operation space of NAS. 
\input{Table/NAS-search-CIFAR10}


Although the models using large circular kernels surpass the counterpart models using large square kernels, the large kernels are not superior to standard $3 \times 3$ kernels as a whole in the manually designed models.
In this subsection, we incorporate the large circular kernels into the advanced gradient-based methods for neural architecture search so as to confirm the proper place of large circular kernels. 
DARTS~\citep{DBLP:conf/iclr/LiuSY19} is the first NAS method based on joint gradient optimization, 
and PC-DARTS~\citep{DBLP:conf/iclr/XuX0CQ0X20} is one of the best gradient-based methods. 
PC-DARTS enables a direct architecture search on ImageNet with only $3.8$ GPU-days while most other NAS methods can only search on CIFAR and then evaluate on ImageNet. 
Hence, we incorporate the convolutions with large circular kernels to the operation space of DARTS and PC-DARTS. Denote our newly searched architectures as DARTS-Circle and PC-DARTS-Circle, respectively. %The complete operation $\mathcal{O}$ is: $3 \times 3$ and $5 \times 5$ separable convolutions, $3 \times 3$ and $5 \times 5$ dilated separable convolutions, $3 \times 3$ max pooling, $3 \times 3$ average pooling, identity, zero, $5 \times 5$ circle separable convolutions and dilated separable convolutions. The last two operations are new for DARTS and PC-DARTS. Our experiments consist of complete architecture search and architecture evaluation.


\input{Table/NAS-search-imagenet}
 
On CIFAR-10, the search and evaluation scenarios simply follow DARTS and PC-DARTS except for some necessary changes for a fair comparison. In the search scenario, the over-parameterized network is constructed by stacking $8$ cells ($6$ normal cells and $2$ reduction cells) for DARTS-Circle and PC-DARTS-Circle, and each cell consists of ${N}={6}$ nodes. In cell $k$, the first $2$ nodes are input nodes, which are the outputs of cells $k - 2$ and $k - 1$, respectively. Each cell's output is the concatenation of all the intermediary nodes. In the evaluation stage, the network comprises $20$ cells ($18$ normal cells and $2$ reduction cells), and each type of cell shares the same architecture. %$B.2$. %~\ref{sec:CIFAR-10-NAS}. \par 




On ImageNet, following DARTS and PC-DARTS, the over-parameterized network starts with three convolution layers of stride 2 to reduce the input image resolution from $224 \times 224$ to $28 \times 28$. The cell architecture is the same with CIFAR-10. To reduce the search time, we randomly sample two subsets from the $1.3\mathrm{M}$ training set of ImageNet, with $10\%$ and $2.5\%$ images, respectively. %The former is used for training the network weights, and the latter is used for updating the hyper-parameters. 
In the evaluation stage, we apply the most popular \textit{mobile setting} where the input image size is fixed to be $224 \times 224$, and the number of multi-add operations does not exceed $600\mathrm{M}$~\citep{DBLP:conf/iclr/LiuSY19,DBLP:conf/iclr/XuX0CQ0X20,chen2019progressive}. %Limited to the mobile setting, we reduce the $14$ stacked cells used in DARTS and PC-DARTS to $13$ stacked cells ($11$ normal cells and $2$ reduction cells) for our models. %See more detailed experimental setup in the Supplementary. %$B.3$. %~\ref{sec:ImageNet-NAS}.
 



The CIFAR-10 results for various convolutional architectures are presented in Table~\ref{NAS-search-CIFAR10}. Notably, both DARTS-Circle and PC-DARTS-Circle outperform the DARTS and PC-DARTS baselines with similar FLOPs, respectively. With AutoAugment~\citep{cubuk2018autoaugment}, PC-DARTS has a surprising performance of $2.15\%$ error rate. However, PC-DARTS-Circle can still boost the performance of PC-DARTS by $+0.13\%$ and achieves a state-of-the-art performance of $2.02\%$ error rate with only $0.1$ GPU-days.


%The ImageNet results and comparison 
The comparisons on ImageNet 
are summarized in Table~\ref{NAS-search-imagenet} and Fig.~\ref{fig:acc_flops}, illustrating that NAS methods have a better trade-off than the strong baseline of manual architecture.
In NAS methods, DARTS-Circle achieves a top-1/5 error of $25.9\%$/$8.1\%$, considerably outperforming the results of $26.7\%$/$8.7\%$ reported by DARTS with similar FLOPs. Limited to the mobile setting, we reduce the $14$ stacked cells used in PC-DARTS-Circle to $13$ stacked cells. 
\input{Figure/acc_flops}
However, PC-DARTS-Circle can still achieve a state-of-the-art top-1/5 error of $24.0\%$/$7.1\%$, slightly outperforming the results of $24.2\%$/$7.3\%$ reported by PC-DARTS. 
When PC-DARTS-Circle uses the same hyper-parameter of 14 stacked cells with PC-DARTS, denoted by PC-DARTS-Circle-v2, the top-1/5 error further reduces to $23.7\%$/$7.0\%$, which is the best result of differentiable architecture search approaches under DARTS-based search space as far as we know. The main difference between PC-DARTS-Circle and PC-DARTS is that the former contains large circular kernels. So we can conclude that large circular kernels are excellent candidates for NAS.
%FairNAS and NSENet report better results with extra modules such as swish activation~\citep{ramachandran2017searching}, SE module~\citep{hu2018squeeze} and AutoAugment~\citep{zoph2020learning}. However, under the fair comparison limited to the mobile setting, our results outperform them.  
It is also worth noting that PC-DARTS-Circle outperforms NSENet, whose operation space contains $27$ traditional operations without convolutions of circular kernels and is much more than the $9$ operations employed in PC-DARTS-Circle. 
%It is also worth noting that PC-DARTS-Circle takes $2.4$ GPU-days for the architecture search, which is significantly less than $3.8$ GPU-days reported by PC-DARTS. It is counter-intuitive because PC-DARTS-Circle contains more operations in its search space. The less search cost could be owning to more efficient parallel optimization for operations and a larger mini-batch of one GPU in our experiment.
\par 

% and is the best known performance to date
%In the past few years, a large body of work has emerged on reducing the amount of calculation and accelerating the search for neural architecture. The search time is reduced to several hours in recent works~\citep{DBLP:conf/cvpr/LiQD0TG20,DBLP:conf/nips/NaymanNRFJZ19,DBLP:conf/iclr/XuX0CQ0X20,DBLP:conf/icml/ZhouYWP19} while the evaluation takes approximately 2 GPU-days on CIFAR-10. It motivates us to sacrifice search efficiency to improve evaluation performance by adding more operations to the operation space. Besides $5 \times 5$ circle separable convolutions and dilated separable convolutions, we consider $7 \times 7$ convolutions, which are employed in NASNet~\citep{zoph2018learning} and AmoebaNet~\citep{real2019regularized} but discarded in methods based on gradient optimization. Because the search time increases linearly with the number of operations, the new search time is still several hours.
\input{Figure/searched_cells_PC_DARTS}

We visualize the searched normal cells and reduction cells of PC-DARTS-Circle on CIFAR-10 (\textit{left}) and ImageNet (\textit{right}) in Fig.~\ref{fig:searched_cells_PC_DARTS}. All other searched cells are shown in the Supplementary. %$D$.   %~\ref{sec:searched-cells}. 
%We observe large circular kernels mainly exist in the reduction cells. According to DARTS~\citep{DBLP:conf/iclr/LiuSY19}, cells located at the $1/3$ and $2/3$ of the total depth of the network are reduction cells, in which all the operations adjacent to the input nodes are of stride two. We speculate that large circular kernels are significant when the size of feature maps change. 
Although large circular kernels only exist in a few layers
and mainly exist in the reduction cells, they have a significant impact on the overall network because the receptive field is stacked as the layers go deeper. 
 



==> Circular Kernel/05Analysis.tex <==
% \subsection{Experimental Setup}
% \label{sec:experiment-setup} 
%We empirically demonstrate the effectiveness of our approach on the image classification task using three standard datasets, CIFAR-10, CIFAR-100, and ImageNet.
%We first show the advantages of large circular kernels by confirmatory experiments on CIFAR-10 and CIFAR-100. Then we compare the $3 \times 3$ circular kernels and the integrated kernels with $3 \times 3$ square kernels on ImageNet in manually designed neural architectures, ResNet-18 and ResNet-50~\citep{he2016deep}. 

For further analysis, we first show the better rotation invariance of large circular kernels compared to large square kernels by the evaluation on rotated or sheared images. Then, by constructing the integrated kernel, we reveal that the circular kernel has an optimization path different from the square kernel. In the Supplementary, %$C$  ~\ref{sec:defor},
we compare convolutions of large circular kernel with deformable convolutions~\citep{jeon2017active,dai2017deformable,zhu2019deformable} in NAS. The searched architecture containing convolutions of large circular kernels is with much less search and evaluation time cost and considerably outperforms the counterpart containing deformable convolutions.


\input{Figure/robustness} 

\subsection{Rotation Invariance of Large Circular Kernels}
%\label{sec:ablation}
%The robustness of CNNs to images with corrupted distributions has become a hot focus of research in recent years. 
To better understand the approximate rotation-invariant property of circular kernels, we investigate their robustness to rotated images or sheared images.  
Specifically, we compare the performance of PC-DARTS-Circle with PC-DARTS searched on CIFAR-10. 
They are both trained on the training set of CIFAR-10 with standard data augmentation.
%, which means that they did not see rotated or sheared images during the training. 
Fig.~\ref{fig:robustness} illustrates the classification errors on the rotated or sheared images generated on the test set of CIFAR-10. 
%PC-DARTS-Circle contains circular kernels and square kernels, denoted by \textit{circle\_square}. PC-DARTS contains square kernels, denoted by \textit{square}. 
The rotation or shear angle range takes the value in $\sD_{e}=\{10, 20, 30, 40, 50, 60, 70, 80\}$. For each angle range $a \in \sD_{e}$, the images are rotated or sheared with an angle uniformly sampled from $\left( -a, a  \right)$, 
and we report the average classification error for three independent tests. \par


We can observe that the advantages of PC-DARTS-Circle steadily increase after $a > 30$, and reach the maximum at $a = 70$, which is roughly $4\%$ for rotation and $5\%$ for shear. The experiments not only justify the better rotation-invariant property of circular kernels, but also reveal that the rotation-invariant property of circular kernels in some layers is helpful to make the overall model more robust to the rotated images or sheared images.


\input{Figure/int_sc}

\subsection{Integrated Kernels and Optimal Path}
\label{sec:3x3-Kernel}

In Section~\ref{transformation}, we %preliminarily proved
analyzed that the model with circular kernels has an optimal path different from that of the model with square kernels during the course of the gradient descent optimization. 
Here, we show their difference empirically by substituting all the $3 \times 3$ square kernels with the corresponding circular kernels or integrated kernels (explained in the followup paragraph) on WRNCifar~\citep{zagoruyko2016wide} and DenseNetCifar~\citep{huang2017densely}. %, and re-train the modified networks on ImageNet. 
%Detailed experimental setup can be found in Supplementary. %$B.1$. %~\ref{sec:CIFAR-10-Artificially}.
\par

We first introduce the integrated kernel in detail. 
Each integrated kernel has two candidate kernels containing a square kernel and a circular kernel, denoted by $\sD = \{\sS,\sR\} $. At each iteration, we randomly select $\sD_p \in \sD $ according to a \textit{binomial} distribution for each convolutional layer. Following~\Eqref{eq.circle_conv} in Section~\ref{sec:method}, we resample the input $\mI$ with a group of offsets denoted by $\{\Delta\vd\}$ that corresponds to each discrete kernel position $\bm{s}$ to form the integrated receptive field.
Then, the output feature map of the corresponding convolution is defined as $\mO_{j} =  \sum_{\bm{s}\in \sS} \mW_{\bm{s}} \mI_{\vj+\bm{s}+\Delta\vd}$. 
% follows:  
% \begin{equation}
%     \mO_{j} =  \sum_{\bm{s}\in \sS} \mW_{\bm{s}} \mI_{\vj+\bm{s}+\Delta\vd}.
% \label{eq.integrated_conv}
% \end{equation}
%In each iteration of training, if $\sD_p=\sS$, all the kernels in one layer are square kernels; %. If $\sD_p=\sR$, all the kernels in one layer become circular kernels. 
%and otherwise circular kernels. \HK{??}
The two types of kernels share the weight matrix but have distinct transformation matrices. During the training, the shared weight matrix is updated at each epoch, but the transformation matrices are randomly picked to determine the type of kernels of each layer at each iteration. \par

We compare the performance of the three versions of kernels on CIFAR-10 and CIFAR-100. %the large dataset of ImageNet. 
The results are presented in Fig.~\ref{fig:int_sc}. %Figure
It is worth noting that the version with integrated kernels yields better results over the other two versions, even though the network architecture is manually designed based on square kernels.
The superiority of the integrated kernels indicates that the switch between circular kernels and square kernels helps the model jump out of the local optima to perform better performance. Consequently, we can conclude 
that the circular kernel has an optimization path different from the square kernel for the gradient descent optimization.   
 




==> Circular Kernel/Figure/3-5-7.tex <==
\begin{figure*}[tb]
    \centering
    %\includegraphics[width=0.7\textwidth]{./Fig/357.pdf}
    \includegraphics[width=0.7\linewidth]{Fig/357.pdf}  
    \caption{The receptive fields and sampling points of circular kernels in size $k \in \{3,5,7\}$. The intersection of dashed lines are the sampling points of square kernels in size $k \in \{3,5,7\}$. All circular receptive fields are concentric and approximately isotropic. A larger circular kernel has a more round receptive field}
    \label{fig:3-5-7}
    %\vspace{-1.8em}%-21pt}%{-10pt}
\end{figure*}

==> Circular Kernel/Figure/acc_flops.tex <==
\begin{wrapfigure}{tbR}{0.5\columnwidth}
\vskip -5pt
	\centering
	\includegraphics[width=0.5\columnwidth]{Fig/acc_flops.pdf}
	%\vspace{-15pt}
	\caption{Comparison of top-1 accuracy on ImageNet with FLOPs (best viewed in color)}
	\label{fig:acc_flops}
	\vskip -5pt
\end{wrapfigure}


==> Circular Kernel/Figure/int_sc.tex <==
\begin{figure*}[t]%[!htb]
\centering
\subfigure[\small{CIFAR-10}]
{\label{fig:ci10}\includegraphics[width=0.41\linewidth]{main_fig/cifar10_s_c_sc.pdf}}
\hspace{10pt}
\subfigure[\small{CIFAR-100}]
{\label{fig:ci100}\includegraphics[width=0.41\linewidth]{main_fig/cifar100_s_c_sc.pdf}}
\caption{Test error ($\%$) of the baselines with square kernels (\textit{Square}) and the corresponding modified versions with circular kernels (\textit{Circle}) or integrated kernels (\textit{Int-SC}) on CIFAR-10 and CIFAR-100 without data augmentation (best viewed in color)}
%\vskip -0.1in
\label{fig:int_sc}
\end{figure*}




==> Circular Kernel/Figure/main_fig.tex <==
\begin{figure*}[tb]%[!htb]
\centering
\subfigure[\small{ResNet}]
{\label{fig:res}\includegraphics[width=0.242\linewidth]{main_fig/cifar10_resnet.pdf}}
\subfigure[\small{VGG}]
{\label{fig:vgg}\includegraphics[width=0.242\linewidth]{main_fig/cifar10_vgg.pdf}}
\subfigure[\small{WRNCifar}]
{\label{fig:wrn}\includegraphics[width=0.242\linewidth]{main_fig/cifar10_wideres.pdf}}
\subfigure[\small{DenseNetCifar}]
{\label{fig:dense}\includegraphics[width=0.242\linewidth]{main_fig/cifar10_densenet.pdf}}\\
\subfigure[\small{ResNet}]{\label{fig:res100}\includegraphics[width=0.242\linewidth]{main_fig/cifar100_resnet.pdf}}
\subfigure[\small{VGG}]{\label{fig:vgg100}\includegraphics[width=0.242\linewidth]{main_fig/cifar100_vgg.pdf}}
\subfigure[\small{WRNCifar}]{\label{fig:wrn100}\includegraphics[width=0.242\linewidth]{main_fig/cifar100_wideres.pdf}}
\subfigure[\small{DenseNetCifar}]{\label{fig:dense100}\includegraphics[width=0.242\linewidth]{main_fig/cifar100_densenet.pdf}}

\caption{Test error ($\%$) of the baselines with square kernels (dashed lines) and the corresponding circular kernel (solid lines) versions in kernel size $k \in \{3,5,7 \}$ on CIFAR-10 (\textit{top}) and CIFAR-100 (\textit{bottom}). For a fair comparison, we use the original data without data augmentation (best viewed in color)}
%\vskip -0.1in
\label{fig:cifar}
\end{figure*}


% \begin{figure*}[!htb]
% \centering
% \subfigure[\small{ResNet}]{\label{fig:res100}\includegraphics[width=0.242\linewidth]{main_fig/cifar100_resnet.pdf}}
% \subfigure[\small{VGG}]{\label{fig:vgg100}\includegraphics[width=0.242\linewidth]{main_fig/cifar100_vgg.pdf}}
% \subfigure[\small{WRNCifar}]{\label{fig:wrn100}\includegraphics[width=0.242\linewidth]{main_fig/cifar100_wideres.pdf}}
% \subfigure[\small{DenseNetCifar}]{\label{fig:dense100}\includegraphics[width=0.242\linewidth]{main_fig/cifar100_densenet.pdf}}
% \vskip -0.1in
% \caption{Test error ($\%$) on CIFAR-100 without data augmentation (best viewed in color)}
% \label{fig:cifar10}
% \end{figure*}

==> Circular Kernel/Figure/robustness.tex <==
% \begin{figure*}[tb]
%     \centering
%     \includegraphics[width=0.9\textwidth]{Fig/robustness.pdf}
%     \vspace{-10pt}
%     \caption{Comparison of classification error of models on rotated and sheared images. }
%     \vspace{-10pt}
%     \label{fig:robustness}
% \end{figure*}

\begin{figure}[ht] %tbp
\centering

% \subfigure[\small{WRNCifar}]{\label{fig:wrn100}\includegraphics[width=0.242\linewidth]{main_fig/cifar100_wideres.pdf}}

\subfigure[\small{Rotation}]
{\label{rotate}\includegraphics[width=0.4\linewidth]{Fig/rotate_robustness.pdf}}
\hspace{10pt}
\subfigure[\small{Shear}]
{\label{shear}\includegraphics[width=0.4\linewidth]{Fig/shear_robustness.pdf}}
%\vspace{-5pt}
\caption{Comparison of classification error on rotated images %or sheared images}
(\textit{left}) or sheared images (\textit{right})}
% \vspace{-1.0em}
\label{fig:robustness}
\end{figure}




% \begin{figtab*}[t]
% 	%\vspace{-7mm}
% \begin{minipage}[t!]{0.4\linewidth}
% 		%\vspace{0mm}
% 		%\centering
% 		\renewcommand\arraystretch{1.1}
% 		\setlength\tabcolsep{1.8mm}
% 		%\footnotesize
% 		%\vspace{-3mm}
%  		\begin{center}
% 			\begin{tabular}{l|c|c|c}
% 				\hline
% 				\multirow{2}*{$\lambda$} & Edges & Params & Flops\\
% 				~ & (N / R) & (M) & (M)\\
% 				\hline
% 				0.2 & 9 / 8 & 5.07 & 580\\
% 				\hline
% 				0.1 & 11 / 6 & 5.88 & 673\\
% 				\hline
% 				0.05 & 13 / 14 & 6.99 & 779\\
% 				\hline
% 			\end{tabular}
% 		\end{center}
% 		%\newline
% 		\vspace{-1mm}
% 		\caption{EnTranNAS-DST with different $\lambda$. ``N'' and ``R'' denote normal and reduction cell, respectively. It is shown that the number of edges is not fixed to access flexible topologies with variant capacities.}
% 		\label{flex}
% 	\end{minipage}\quad\ \
% 	%\vspace{8mm}
	
% 	\begin{minipage}[t!]{0.50\linewidth}
% 		\centering
% 		%\hspace{6mm}
% 		\vspace{-1mm}
% 		\includegraphics[width=1.\linewidth]{Fig/robustness.pdf}
% 		%\vspace{-2.83mm}
% 		\figcaption{Comparison of top-1 accuracies on ImageNet with parameters (left) and Flops (right). Zoom in to view better.}
% 		\label{curve}
% 	\end{minipage}
% % \begin{minipage}[t!]{0.57\linewidth}
% % \centering
% % \includegraphics[width=1\linewidth]{Fig/robustness.pdf}
% % %\vspace{-15pt}
% % %\caption{Test error to rotated images}
% % \figcaption{Comparison of classification error on rotated or sheared images.}
% % \vspace{-5pt}
% % \label{fig:robustness}
% % \end{minipage}
% 	%\vspace{-4mm}
% \end{figtab*}






% \begin{figure*}[tb]
% \centering
% \begin{minipage}{0.38\textwidth}
% \includegraphics[width=1\linewidth]{Fig/rotate_robustness.pdf}
% \vspace{-15pt}
% \label{rotate}
% %\caption{Test error to rotated images}
% \end{minipage}
% \hspace{15pt}
% \begin{minipage}{0.38\textwidth}
% %\flushright
% \includegraphics[width=1\linewidth]{Fig/shear_robustness.pdf}
% \vspace{-15pt}
% \label{shear}
% %\caption{Test error to sheared images}
% \end{minipage}
% \caption{Comparison of classification error on rotated or sheared images.}
% \vspace{-5pt}
% \label{fig:robustness}
% \end{figure*}

==> Circular Kernel/Figure/robustness_original.tex <==
\begin{figure*}[tb]
    \centering
    \includegraphics[width=0.9\textwidth]{Fig/robustness.pdf}
    \vspace{-10pt}
    \caption{Comparison of classification error of models on rotated and sheared images}
    \vspace{-10pt}
    \label{fig:robustness}
\end{figure*}

==> Circular Kernel/Figure/searched_cells_PC_DARTS.tex <==
\begin{figure*}[tb]
\centering
\subfigure[The normal cell on CIFAR-10]{\label{pc_im_ncells_s1}\includegraphics[width=0.42\linewidth]{Fig/cifar_n.pdf}}
\hspace{0.2em}
\subfigure[The normal cell on ImageNet]{\label{pc_im_ncells_s3}\includegraphics[width=0.42\linewidth]{Fig/imagenet_n.pdf}}
\subfigure[The reduction cell on CIFAR-10]{\label{pc_im_ncells_s2}\includegraphics[width=0.42\linewidth]{Fig/cifar_r.pdf}}
\hspace{0.2em}
\subfigure[The reduction cell on ImageNet]{\label{pc_im_ncells_s4}\includegraphics[width=0.42\linewidth]{Fig/imagenet_r.pdf}}
%\vspace{-0.2em}
\caption{The searched normal cells and reduction cells of PC-DARTS-Circle on CIFAR-10 (\textit{left}) and ImageNet (\textit{right}). The circular kernels are marked in \red{red}}
\vspace{-0.5em}  %-5pt}
\label{fig:searched_cells_PC_DARTS}
\end{figure*}

==> Circular Kernel/Figure/searched_cells_cifar.tex <==
\begin{figure*}[!htb]
\centering
\subfigure[The normal cell of PC-DARTS]{\includegraphics[width=0.45\linewidth]{Fig/P_cifar_n.pdf}}
\hspace{0.2em}
\subfigure[The normal cell of PC-DARTS-Circle]{\includegraphics[width=0.45\linewidth]{Fig/cifar_n.pdf}}
\subfigure[The reduction cell of PC-DARTS]{\includegraphics[width=0.45\linewidth]{Fig/P_cifar_r.pdf}}
\hspace{0.2em}
\subfigure[The reduction cell of PC-DARTS-Circle]{\includegraphics[width=0.45\linewidth]{Fig/cifar_r.pdf}}

\caption{The searched normal and reduction cells of PC-DARTS (\textit{left}) and PC-DARTS-Circle (\textit{right}) on CIFAR-10. The large circular kernel is marked in \red{red}}
%\vspace{-0.5em}  %-5pt}
\label{fig:cells_cifar}
\end{figure*}


 
% \begin{figure*}[tb]%[tb]
% \centering
% \begin{minipage}{0.50\textwidth}
% \subfloat[The normal cell found by PC-DARTS]{\includegraphics[width=1.0\linewidth]{Fig/P_cifar_n.pdf}}\label{pc_ncells_s1}\\

% \subfloat[The reduction cell found by PC-DARTS]{\includegraphics[width=1.0\linewidth]{Fig/P_cifar_r.pdf}}\label{pc_ncells_s2}
% \end{minipage}
% \begin{minipage}{0.46\textwidth}
% \subfloat[The normal cell found by PC-DARTS-Circle]{\includegraphics[width=1.0\linewidth]{Fig/cifar_n.pdf}}\label{pc_ncells_s3}\\
% \begin{center}
% \vspace{-0.5em}
% \subfloat[The reduction cell found by PC-DARTS-Circle]{\includegraphics[width=1.0\linewidth]{Fig/cifar_r.pdf}}\label{pc_ncells_s4}
% \end{center}
% \end{minipage}
% \caption{The searched normal and reduction cells of PC-DARTS (left-hand side) and PC-DARTS-Circle (right-hand side) on CIFAR-10. The large circular kernel is marked in \red{red}.}
% \label{fig:cells_cifar}
% \end{figure*}

==> Circular Kernel/Figure/searched_cells_darts.tex <==
\begin{figure*}[!htb]
\centering
\subfigure[The normal cell of DARTS]{\includegraphics[width=0.45\linewidth]{Fig/d_c_n.pdf}}
\hspace{0.2em}
\subfigure[The normal cell of DARTS-Circle]{\includegraphics[width=0.45\linewidth]{Fig/d_cs_n.pdf}}
\subfigure[The reduction cell of DARTS]{\includegraphics[width=0.45\linewidth]{Fig/d_c_r.pdf}}
\hspace{0.2em}
\subfigure[The reduction cell of DARTS-Circle]{\includegraphics[width=0.45\linewidth]{Fig/d_cs_r.pdf}}
\caption{The searched normal and reduction cells of DARTS (\textit{left}) and DARTS-Circle (\textit{right}) on CIFAR-10. The large circular kernels are marked in \red{red}}
%\vspace{-0.5em}  %-5pt}
\label{fig:cells_darts}
\end{figure*}



% \begin{figure*}[tb]%[tb]
% \centering
% \begin{minipage}{0.49\textwidth}
% \subfloat[The normal cell found by DARTS]{\includegraphics[width=1.0\linewidth]{Fig/d_c_n.pdf}}\label{ncells_s1}\\
% %\vspace{0.4em}
% \subfloat[The reduction cell found by DARTS]{\includegraphics[width=1.0\linewidth]{Fig/d_c_r.pdf}}\label{ncells_s2}
% \end{minipage}
% \begin{minipage}{0.49\textwidth}
% \subfloat[The normal cell found by DARTS-Circle]{\includegraphics[width=1.0\linewidth]{Fig/d_cs_n.pdf}}\label{ncells_s3}\\
% \vspace{0.4em}
% \begin{center}
% \subfloat[The reduction cell found by DARTS-Circle]{\includegraphics[width=1.0\linewidth]{Fig/d_cs_r.pdf}}\label{ncells_s4}
% \end{center}
% \end{minipage}
% \caption{The searched normal and reduction cells of DARTS (left-hand side) and DARTS-Circle (right-hand side) on CIFAR-10. The large circular kernels are marked in \red{red}.}
% \label{fig:cells_darts}
% \end{figure*}

==> Circular Kernel/Figure/searched_cells_imagenet.tex <==
\begin{figure*}[!htb]
\centering
\subfigure[The normal cell of PC-DARTS]{\includegraphics[width=0.45\linewidth]{Fig/P_imagenet_n.pdf}}
\hspace{0.2em}
\subfigure[The normal cell of PC-DARTS-Circle]{\includegraphics[width=0.45\linewidth]{Fig/imagenet_n.pdf}}
\subfigure[The reduction cell of PC-DARTS]{\includegraphics[width=0.45\linewidth]{Fig/P_imagenet_r.pdf}}
\hspace{0.2em}
\subfigure[The reduction cell of PC-DARTS-Circle]{\includegraphics[width=0.45\linewidth]{Fig/imagenet_r.pdf}}

\caption{The searched normal and reduction cells of PC-DARTS (\textit{left}) and PC-DARTS-Circle (\textit{right}) on ImageNet. The large circular kernels are marked in \red{red}}
\label{fig:cells_imagenet}
\end{figure*}











% \begin{figure*}[tb]%[tb]  %%[!ht]%
% \centering
% \begin{minipage}{0.48\textwidth}
% \subfloat[The normal cell found by PC-DARTS]{\includegraphics[width=1.0\linewidth]{Fig/P_imagenet_n.pdf}}\label{ncells_s1}\\
% \vspace{-0.9em}
% \subfloat[The reduction cell found by PC-DARTS]{\includegraphics[width=1.0\linewidth]{Fig/P_imagenet_r.pdf}}\label{ncells_s2}
% \end{minipage}
% \begin{minipage}{0.45\textwidth}
% \subfloat[The normal cell found by PC-DARTS-Circle]{\includegraphics[width=1.0\linewidth]{Fig/imagenet_n.pdf}}\label{ncells_s3}\\
% %\vspace{0.6em}
% \begin{center}
% \subfloat[The reduction cell found by PC-DARTS-Circle]{\includegraphics[width=1.0\linewidth]{Fig/imagenet_r.pdf}}\label{ncells_dv2}
% \end{center}
% \end{minipage}
% \caption{The searched normal and reduction cells of PC-DARTS (left-hand side) and PC-DARTS-Circle (right-hand side) on ImageNet. The large circular kernels are marked in \red{red}.}
% \vspace{-1em}%-5pt}
% \label{fig:cells_imagenet}
% \end{figure*}

==> Circular Kernel/Figure/square-circle.tex <==
\begin{figure*}[tb]
    \centering
    \includegraphics[width=0.75\textwidth]{Fig/square_to_circle.pdf}
    \vspace{-15pt}
    \caption{Approximation of a $3 \times 3$ circular kernel on a $3 \times 3$ square kernel 
    %\HK{fix (b): Receptive field of a circular kernel }
    }
    %\vspace{-5pt}
    \label{fig:square-circle}
\end{figure*}

==> Circular Kernel/Table/NAS-search-CIFAR10.tex <==
\begin{table*}[t]
\centering
\caption{Comparison with state-of-the-art searched network architectures on CIFAR-10. $\ddagger$ denotes
model trained with AutoAugment~\cite{cubuk2018autoaugment}}
%\tiny
\small
\begin{threeparttable}[b]
\resizebox{0.8\textwidth}{!}{

\begin{tabular}{@{}lcccccc@{}}
\toprule
\multirow{2}{*}{\textbf{Architecture}} & \textbf{Test Err.} & \textbf{Params} & \textbf{Search Cost} & \multirow{2}{*}{\textbf{Search Method}} \\
&                            \textbf{(\%)} & \textbf{(M)} & \textbf{(GPU-days)} &\\
\midrule
DenseNet-BC~\cite{huang2017densely}                       & 3.46  & 25.6 & -    & manual \\
\midrule
NASNet-A + cutout~\cite{zoph2018learning}                 & 2.65  & 3.3  & 1800 & RL      \\
%ENAS + cutout~\cite{pham2018efficient}                    & 2.89 & 4.6  & 0.5  & RL \\
AmoebaNet-A + cutout~\cite{real2019regularized}          & 3.34$\pm$0.06 &  3.2  & 3150 & evolution \\
AmoebaNet-B + cutout~\cite{real2019regularized}           & 2.55$\pm$0.05 & 2.8  & 3150 & evolution \\
% Hireachical Evolution~\cite{liu2017hierarchical}          & 3.75$\pm$0.12 &  15.7 & 300  & evolution \\
 
\midrule
%ProxylessNAS + cutout~\cite{cai2018proxylessnas}   & 2.08 & -     &  4.0    & gradient-based \\
P-DARTS + cutout~\cite{chen2019progressive}      & 2.50 &  3.4  & 0.3 & gradient-based \\
%BayesNAS + cutout~\cite{zhou2019bayesnas}        & 2.81$\pm$0.04 &  3.4  & 0.2& gradient-based \\
R-DARTS(L2) + cutout~\cite{bender2018understanding} & 2.95$\pm$0.21 & - & 1.6 & gradient-based \\
S-DARTS-ADV + cutout~\cite{DBLP:conf/icml/ChenH20} & 2.61$\pm$0.02 & 3.3 & 1.3 & gradient-based \\
Fair DARTS + cutout~\cite{chu2020fair} & 2.54$\pm$0.05 & 3.3 & - & gradient-based \\
EnTranNAS-DST + cutout~\cite{yang2021towards}  &2.48$\pm$0.08&3.2&0.1& gradient-based\\
DARTS$-$ + cutout~\cite{DBLP:conf/iclr/ChuW0LWY21} & 2.59$\pm$0.08 & 3.5 & 0.4 & gradient-based\\
\midrule
DARTS + cutout~\cite{DBLP:conf/iclr/LiuSY19}          & 2.76$\pm$0.09 &  3.3 & 0.4 & gradient-based \\
%PC-DARTS + cutout~\cite{DBLP:conf/iclr/XuX0CQ0X20} &2.57$\pm$0.07 & 3.6  & 0.1& gradient-based \\
PC-DARTS + cutout$^\ddagger$~\cite{DBLP:conf/iclr/XuX0CQ0X20} &2.15$\pm$0.04 & 3.6  & 0.1& gradient-based \\
\midrule
\midrule
DARTS-Circle + cutout    & 2.62$\pm$0.08 &  3.9 & 0.4 & gradient-based \\
%PC-DARTS-Circle + cutout & 2.54$\pm$0.07 & 3.5  & 0.1& gradient-based \\
PC-DARTS-Circle + cutout$^\ddagger$ & 2.02$\pm$0.05 & 3.5  & 0.1& gradient-based \\
\bottomrule
\end{tabular}
}
\end{threeparttable}
% \vspace{-5pt}

% \vspace{-1.5em}
\label{NAS-search-CIFAR10}
\end{table*}

==> Circular Kernel/Table/NAS-search-imagenet.tex <==
\begin{table*}[tb]
\centering
\caption{Comparison with state-of-the-art searched architectures on ImageNet (\textbf{mobile setting}). $\ddagger$: These architectures are searched on ImageNet directly, others are searched on CIFAR-10 or CIFAR-100 and transferred to ImageNet}

\begin{threeparttable}[b]
\resizebox{0.9\textwidth}{!}{
\begin{tabular}{@{}lcccccc@{}}
\toprule
\multirow{2}{*}{\textbf{Architecture}} & \multicolumn{2}{c}{\textbf{Test Err. (\%)}} & \textbf{Params} & \textbf{FLOPs} & \textbf{Search Cost} & \multirow{2}{*}{\textbf{Search Method}} \\% $\times+$  
\cmidrule(lr){2-3}
&                            \textbf{top-1} & \textbf{top-5} & \textbf{(M)} & \textbf{(M)} & \textbf{(GPU-days)} &\\
\midrule
ResNet50~\cite{he2016deep} & 24.7 &-& 25.6 &4100 & - & manual \\
Inception-v1~\cite{szegedy2015going}          & 30.2 & 10.1 & 6.6  & 1448 &-    & manual \\
MobileNet~\cite{howard2017mobilenets}         & 29.4 & 10.5 & 4.2   & 569  &-    & manual \\
%ShuffleNet 2$\times$ (v1)~\cite{zhang2018shufflenet} & 26.4 & 10.2 & $\sim$5    &524  & -    & manual \\
ShuffleNet 2$\times$ (v2)~\cite{ma2018shufflenet}    & 25.1 & - & $\sim$5    & 591  &-    & manual \\
\midrule
NASNet-A~\cite{zoph2018learning}              & 26.0 & 8.4  & 5.3   & 564  &1800 & RL \\
%AmoebaNet-A~\cite{real2019regularized}        & 25.5 & 8.0  & 5.1   & 3150 & evolution \\
%MnasNet-92~\cite{tan2018mnasnet}              & 25.2 & 8.0  & 4.4   &388  & -    & RL \\
AmoebaNet-C~\cite{real2019regularized}        & 24.3 & 7.6  & 6.4   & 570  &3150 & evolution \\
FairNAS-A~\cite{chu2019fairnas}               & 24.7 &  -   & 4.6    & 388  & 12    &evolution \\  %  +x  388
%BN-NAS~\cite{chen2021bn} (ImageNet)$^\ddagger$ & 24.3 &  -   & 5.4    &  0.8    &evolution \\  % +x 470
\midrule
%ProxylessNAS (ImageNet)$^\ddagger$~\cite{cai2018proxylessnas}       & 24.9 & 7.5  & 7.1   & 465  & 8.3  & gradient-based \\
P-DARTS~\cite{chen2019progressive}                 & 24.4 & 7.4  & 4.9   & 557  & 0.3  & gradient-based \\
S-DARTS-ADV~\cite{DBLP:conf/icml/ChenH20}&25.2 & 7.8 & -&- & -&gradient-based \\
Fair DARTS~\cite{chu2020fair}$^\ddagger$ &24.4 &7.4 & 4.3&440&3.0&gradient-based \\
%BayesNAS~\cite{zhou2019bayesnas}                         & 26.5 & 8.9  & 3.9  & -  & 0.2  & gradient-based \\
NSENet~\cite{ci2020evolving}                         & 24.5 & -  & 4.6   & 330&-  & gradient-based \\ % +x 330
\midrule

DARTS~\cite{DBLP:conf/iclr/LiuSY19}      & 26.7 & 8.7  & 4.7   & 574  &0.4    & gradient-based \\
PC-DARTS (CIFAR-10)~\cite{DBLP:conf/iclr/XuX0CQ0X20} &25.1&7.8&5.3& 586 & 0.1 & gradient-based \\
PC-DARTS (ImageNet)$^\ddagger$~\cite{DBLP:conf/iclr/XuX0CQ0X20}  & 24.2 &7.3  & 5.3  & 597  & 3.2 & gradient-based \\ 
\midrule
\midrule
DARTS-Circle      & 25.9 & 8.1  & 5.3   & 583    & 0.4 & gradient-based \\ 
PC-DARTS-Circle (CIFAR-10) &24.9&7.7&5.0&571&0.1&gradient-based \\
PC-DARTS-Circle (ImageNet)$^\ddagger$ &  24.0  &  7.1  & 5.5  & 599 & 3.2 & gradient-based \\ 
PC-DARTS-Circle-v2 (ImageNet)$^\ddagger$ &  23.7  &  7.0  & 5.7  & 639 & 3.2 & gradient-based \\ 
\bottomrule			
\end{tabular}}
%\begin{tablenotes}
%\item[$\ddagger$] {\footnotesize These architectures are searched on ImageNet directly, others are searched on CIFAR-10 or CIFAR-100 \\and transferred to ImageNet. } 
%\end{tablenotes}
\end{threeparttable}
% \vspace{-5pt}

%\vspace{-5pt}
\label{NAS-search-imagenet}
\end{table*}





% \begin{table}[t]
% \centering
% \caption{Comparison with state-of-the-art architectures on ImageNet (mobile setting).}
% \label{NAS-search-imagenet}
% \begin{threeparttable}[b]
% \resizebox{\textwidth}{!}{
% \begin{tabular}{@{}lcccccc@{}}
% \toprule
% \multirow{2}{*}{\textbf{Architecture}} & \multicolumn{2}{c}{\textbf{Test Err. (\%)}} & \textbf{Params} & $\times+$ & \textbf{Search Cost} & \multirow{2}{*}{\textbf{Search Method}} \\
% \cmidrule(lr){2-3}
% &                            \textbf{top-1} & \textbf{top-5} & \textbf{(M)} & \textbf{(M)} & \textbf{(GPU-days)} &\\
% \midrule
% Inception-v1~\cite{szegedy2015going}          & 30.2 & 10.1 & 6.6 & 1448 & -    & manual \\
% MobileNet~\cite{howard2017mobilenets}         & 29.4 & 10.5 & 4.2 & 569  & -    & manual \\
% ShuffleNet 2$\times$ (v1)~\cite{zhang2018shufflenet} & 26.4 & 10.2 & $\sim$5  & 524  & -    & manual \\
% ShuffleNet 2$\times$ (v2)~\cite{ma2018shufflenet}    & 25.1 & - & $\sim$5  & 591  & -    & manual \\
% \midrule
% NASNet-A~\cite{zoph2018learning}              & 26.0 & 8.4  & 5.3 & 564  & 1800 & RL \\
% AmoebaNet-A~\cite{real2019regularized}        & 25.5 & 8.0  & 5.1 & 555  & 3150 & evolution \\
% AmoebaNet-C~\cite{real2019regularized}        & 24.3 & 7.6  & 6.4 & 570  & 3150 & evolution \\
% MnasNet-92~\cite{tan2018mnasnet}              & 25.2 & 8.0  & 4.4 & 388  & -    & RL \\
% \midrule
% DARTS~\cite{DBLP:conf/iclr/LiuSY19}      & 26.7 & 8.7  & 4.7 & 574  & 4.0    & gradient-based \\
% ProxylessNAS (ImageNet)$^\ddagger$~\cite{cai2018proxylessnas}       & 24.9 & 7.5  & 7.1 & 465  & 8.3  & gradient-based \\
% P-DARTS~\cite{chen2019progressive}                 & 24.4 & 7.4  & 4.9 & 557  & 0.3  & gradient-based \\
% BayesNAS~\cite{zhou2019bayesnas}                         & 26.5 & 8.9  & 3.9 & -  & 0.2  & gradient-based \\
% PC-DARTS (ImageNet)$^\ddagger$~\cite{DBLP:conf/iclr/XuX0CQ0X20}       & 24.2 &7.3  & 5.3 & 597  & 3.8 & gradient-based \\ 
% \midrule
% PC-DARTS-Circle (ImageNet)$^\ddagger$ & -  & -  & - & -  & - & gradient-based \\ 
% \bottomrule			
% \end{tabular}
% }
% \begin{tablenotes}
% \item[$\ddagger$] {\footnotesize This architecture was searched on ImageNet directly, otherwise it was searched on CIFAR10 or CIFAR100.}
% \end{tablenotes}
% \end{threeparttable}
% %\vspace{-5pt}
% \end{table}

==> Circular Kernel/Table/int_sc.tex <==
\begin{table}[tb]
\centering
\caption{Test error ($\%$) of the baselines with square kernels (\textit{Square}) and the corresponding modified versions with circular kernels (\textit{Circle}) or integrated kernels (\textit{Int-SC}) on CIFAR-10 and CIFAR-100. 
%\textit{Square} and \textit{Circle} respectively indicate the existing CNNs with square kernels and the counterpart CNNs with circular kernels. \textit{Int-SC} indicates the integration of square and circular kernels. 
We run the model $5$ times for each dataset \& model setting to reduce the variance}
\small
\begin{threeparttable}[b]
%\resizebox{0.48\textwidth}{!}{
\begin{tabular}{lccc}
\toprule
\textbf{Model}&\textbf{Kernel}&\textbf{CIFAR-10}&\textbf{CIFAR-100}\\
%\cmidrule(lr){2-3}\cmidrule(lr){4-5} 
%&WRNCifar&DenseNetCifar&WRNCifar&DenseNetCifar\\
\midrule  
WRNCifar&{Square}      &$  4.33\pm0.10 $&$ 20.59\pm0.16  $ \\
WRNCifar&{Circle}      &$  4.44\pm0.12 $&$ 20.89\pm0.22  $ \\
WRNCifar&{Int-SC}      &$  4.20\pm0.11 $&$ 20.48\pm0.12  $ \\ 
\midrule  
DenseNetCifar&{Square}      &$  5.26\pm0.11 $&$ 23.07\pm0.22  $ \\
DenseNetCifar&{Circle}      &$  5.32\pm0.09 $&$ 23.04\pm0.18  $ \\
DenseNetCifar&{Int-SC}      &$  5.06\pm0.04 $&$ 22.91\pm0.16  $ \\ 
\bottomrule
\end{tabular}
%}
\end{threeparttable}
%\vspace{-5pt}

\label{table:int_sc}
% \vspace{-5pt}
% \vskip -0.1in
\end{table}




% \begin{table*}[tb]
% \centering
% \begin{threeparttable}[b]
% \resizebox{0.8\textwidth}{!}{
% \begin{tabular}{lcccc}
% \toprule
% \multirow{2}{*}{\textbf{Model}}&\multicolumn{2}{c}{\textbf{CIFAR-10}}&\multicolumn{2}{c}{\textbf{CIFAR-100}}\\
% \cmidrule(lr){2-3}\cmidrule(lr){4-5} 
% &WRNCifar&DenseNetCifar&WRNCifar&DenseNetCifar\\
% \midrule  
% {Square}      &$  4.20\pm0.07 $&$ 4.25\pm0.10  $ &$ 20.59\pm0.18 $&$ 21.08\pm0.32 $\\
% {Circle}      &$  4.58\pm0.11 $&$ 4.39\pm0.17  $ &$ 21.25\pm0.14 $&$ 21.17\pm0.12 $\\
% {Int-SC}      &$  5.17\pm0.13 $&$ 4.86\pm0.09  $ &$ 22.45\pm0.15 $&$ 21.89\pm0.18 $\\ 
% \bottomrule
% \end{tabular}
% }
% \end{threeparttable}
% \vspace{-5pt}
% \caption{Test error ($\%$) of the baselines with square kernels (Square) and the corresponding circular kernel (Circle) versions in kernel size $k \in \{3,5,7 \}$ on CIFAR-10 and CIFAR-100. We run the model $5$ times for each dataset \& model setting to reduce the variance. With the increment of kernel size, the advantage of circular kernel over square kernel becomes more distinct.}
% \label{int_sc}
% %\vskip -0.1in
% \end{table*}









==> Circular Kernel/Table/large-circular-kernel.tex <==
\begin{table*}[htbp]
\centering
\caption{Test error ($\%$) of the baselines with square kernels (Square) and the corresponding circular kernel (Circle) versions in kernel size $k \in \{3,5,7 \}$ on CIFAR-10 and CIFAR-100. For a fair comparison, we use the original data without data augmentation. We run the model $5$ times for each dataset \& model setting to reduce the variance}
\begin{threeparttable}[b]
\resizebox{0.85\textwidth}{!}{
\begin{tabular}{lccrccr}
\toprule
\multirow{2}{*}{\textbf{Model}}&\multicolumn{3}{c}{\textbf{CIFAR-10}}&\multicolumn{3}{c}{\textbf{CIFAR-100}}\\
\cmidrule(lr){2-4}\cmidrule(lr){5-7} 
&Square&Circle&Test Err.$\downarrow$&Square&Circle&Test Err.$\downarrow$\\
\midrule

VGG ($3 \times 3$) &$  10.75
\pm0.10 $&$ 10.40\pm0.31 $&$\textbf{\BLUE{0.35}}$ 
&$ 36.39\pm0.15 $&$ 34.74\pm0.09 $&$\textbf{\BLUE{1.65}}$\\

VGG ($5 \times 5$) &$ 11.27\pm0.22 $&$ 9.79\pm0.23 $&$\textbf{\BLUE{1.48}}$ 
&$ 37.92\pm0.43 $&$ 34.61\pm0.20 $&$\textbf{\BLUE{3.31}}$\\

VGG ($7 \times 7$) &$  12.78\pm0.11 $&$ 11.24\pm0.32  $&$\textbf{\BLUE{1.54}}$ 
&$ 40.97\pm0.24 $&$ 37.46\pm0.16 $&$\textbf{\BLUE{3.51}}$\\ 
\midrule

ResNet ($3 \times 3$)&$  11.22\pm0.16 $&$ 10.72\pm0.21 $&$\textbf{\BLUE{0.50}}$ 
&$ 42.45\pm0.43 $&$ 40.03\pm0.35 $&$\textbf{\BLUE{2.42}}$\\
ResNet ($5 \times 5$)&$  12.97\pm0.25 $&$ 11.42\pm0.13 $&$\textbf{\BLUE{1.55}}$ 
&$ 43.67\pm0.53 $&$ 41.28\pm0.19 $&$\textbf{\BLUE{2.39}}$\\
ResNet ($7 \times 7$)&$  14.51\pm0.35 $&$ 12.27\pm0.47 $&$\textbf{\BLUE{2.24}}$
&$ 46.89\pm0.11 $&$ 41.53\pm0.67 $&$\textbf{\BLUE{5.36}}$\\
\midrule

WRNCifar ($3 \times 3$)  
&$  14.13\pm0.06 $&$ 11.70\pm0.52  $&$\textbf{\BLUE{2.43}}$ 
&$ 33.34\pm0.48 $&$ 32.99\pm0.57 $&$\textbf{\BLUE{0.35}}$\\
WRNCifar ($5 \times 5$)     
&$ 12.92\pm0.40 $&$ 10.39\pm0.39  $&$\textbf{\BLUE{2.53}}$ 
&$ 36.51\pm0.13 $&$ 34.38\pm0.10 $&$\textbf{\BLUE{2.13}}$\\
WRNCifar ($7 \times 7$) 
&$  10.70\pm0.08 $&$ 8.73\pm0.22  $&$\textbf{\BLUE{1.97}}$ 
&$ 39.97\pm0.33 $&$ 36.81\pm0.64 $&$\textbf{\BLUE{3.16}}$\\ 
\midrule
DenseNetCifar ($3 \times 3$)
&$  8.41\pm0.08 $&$ 8.30\pm0.42 $&$\textbf{\BLUE{0.11}}$ 
&$ 30.83\pm0.28 $&$ 29.72\pm0.50 $&$\textbf{\BLUE{1.11}}$\\
DenseNetCifar ($5 \times 5$)
&$  8.59\pm0.18 $&$ 7.94\pm0.07 $&$\textbf{\BLUE{0.65}}$ 
&$ 30.84\pm0.10 $&$ 29.26\pm0.20 $&$\textbf{\BLUE{1.58}}$\\
DenseNetCifar ($7 \times 7$)
&$  8.92\pm0.06 $&$ 7.93\pm0.01 $&$\textbf{\BLUE{0.99}}$
&$ 32.53\pm0.62 $&$ 29.81\pm0.32 $&$\textbf{\BLUE{2.72}}$\\
\bottomrule
\end{tabular}
}
\end{threeparttable}
% \vspace{-5pt}
% With the increment of kernel size, the advantage of circular kernel over square kernel becomes more distinct.}
\label{large-circular-kernel}
%\vskip -0.1in
\end{table*}



==> Circular Kernel/Table/large_circular_cifar.tex <==
\begin{table*}[tb]
\centering
\caption{Test error ($\%$) of the baselines with square kernels (Square) and the corresponding circular kernel (Circle) versions in kernel size $k \in \{3,5,7 \}$ on CIFAR-10 and CIFAR-100. With the increment of kernel size, the advantage of circular kernel over square kernel becomes more distinct}
\label{large-circular-kernel-aug}

\begin{threeparttable}[b]
\resizebox{\textwidth}{!}{
\begin{tabular}{lccrccr}
\toprule
\multirow{2}{*}{\textbf{Model}}&\multicolumn{3}{c}{\textbf{CIFAR-10}}&\multicolumn{3}{c}{\textbf{CIFAR-100}}\\
\cmidrule(lr){2-4}\cmidrule(lr){5-7} 
&Square&Circle&Test Err.$\downarrow$&Square&Circle&Test Err.$\downarrow$\\
\midrule
VGG ($3 \times 3$) &$  5.91
\pm0.04 $&$ 5.81\pm0.21 $&$\textbf{\BLUE{0.10}}$ 
&$ 25.19\pm0.12 $&$ 25.10\pm0.10 $&$\textbf{\BLUE{0.09}}$\\

VGG ($5 \times 5$) &$ 6.96\pm0.21 $&$ 6.72\pm0.11 $&$\textbf{\BLUE{0.24}}$ 
&$ 28.08\pm0.29 $&$ 28.02\pm0.06 $&$\textbf{\BLUE{0.06}}$\\

VGG ($7 \times 7$) &$  7.77\pm0.06 $&$ 7.62\pm0.09  $&$\textbf{\BLUE{0.15}}$ 
&$ 30.59\pm0.29 $&$ 29.99\pm0.32 $&$\textbf{\BLUE{0.60}}$\\ 
\midrule

ResNet ($3 \times 3$)&$  5.75\pm0.03 $&$ 5.74\pm0.06 $&$\textbf{\BLUE{0.01}}$ 
&$ 27.47\pm0.19 $&$ 27.56\pm0.09 $&$\textbf{\BLUE{-0.09}}$\\
ResNet ($5 \times 5$)&$  6.33\pm0.07 $&$ 6.13\pm0.16 $&$\textbf{\BLUE{0.20}}$ 
&$ 28.00\pm0.41 $&$ 27.87\pm0.26 $&$\textbf{\BLUE{0.13}}$\\
ResNet ($7 \times 7$)&$  6.82\pm0.35 $&$ 6.62\pm0.07 $&$\textbf{\BLUE{0.20}}$
&$ 29.11\pm0.25 $&$ 28.27\pm0.03 $&$\textbf{\BLUE{0.84}}$\\

\midrule  

WRNCifar ($3 \times 3$)     &$  4.21\pm0.06 $&$ 4.25\pm0.09  $&$\textbf{\BLUE{-0.04}}$ &$ 20.59\pm0.18 $&$ 21.10\pm0.32 $&$\textbf{\BLUE{-0.51}}$\\
WRNCifar ($5 \times 5$)     &$  4.58\pm0.14 $&$ 4.39\pm0.18  $&$\textbf{\BLUE{0.19}}$ &$ 21.24\pm0.14 $&$ 21.16\pm0.12 $&$\textbf{\BLUE{0.08}}$\\
WRNCifar ($7 \times 7$)     &$  5.18\pm0.16 $&$ 4.87\pm0.06  $&$\textbf{\BLUE{0.31}}$ &$ 22.44\pm0.15 $&$ 21.91\pm0.18 $&$\textbf{\BLUE{0.53}}$\\ 
\midrule
DenseNetCifar ($3 \times 3$)&$  5.05\pm0.11 $&$ 5.20\pm0.09 $&$\textbf{\BLUE{-0.15}}$ &$ 22.76\pm0.20 $&$ 22.62\pm0.17 $&$\textbf{\BLUE{0.14}}$\\
DenseNetCifar ($5 \times 5$)&$  5.19\pm0.12 $&$ 5.15\pm0.11 $&$\textbf{\BLUE{0.04}}$ &$ 23.31\pm0.41 $&$ 22.96\pm0.16 $&$\textbf{\BLUE{0.35}}$\\
DenseNetCifar ($7 \times 7$)&$  5.47\pm0.34 $&$ 5.36\pm0.03 $&$\textbf{\BLUE{0.11}}$&$ 23.64\pm0.19 $&$ 23.26\pm0.10 $&$\textbf{\BLUE{0.38}}$\\
\bottomrule
\end{tabular}
}
\end{threeparttable}

%\vskip -0.05in
\end{table*}



==> Circular Kernel/Table/offset_vs_circle.tex <==
\begin{table*}[ht]
\centering
\caption{Comparison with searched network architecture containing deformable convolutions (PC-DARTS-Deformable) on CIFAR-10}
\begin{threeparttable}[b]
\resizebox{0.8\textwidth}{!}{
\begin{tabular}{@{}lcccccc@{}}
\toprule
\multirow{2}{*}{\textbf{Architecture}} & \textbf{Test Err.} & \textbf{Params} & \textbf{Search Cost} & \textbf{Evaluation Cost} \\
&                            \textbf{(\%)} & \textbf{(M)} & \textbf{(GPU-days)} &\textbf{(GPU-days)}\\
\midrule
PC-DARTS-Deformable + cutout & 4.28 & 5.7  & 0.7& 4.8 \\
PC-DARTS-Circle + cutout & 2.54 & 3.5  & 0.1& 1.4 \\
\bottomrule
\end{tabular}
}
\end{threeparttable}
\vspace{-5pt}

\label{NAS-search-defor}
\end{table*}

==> Circular Kernel/math_commands.tex <==
%%%%%%%%%%%%%%%%%%%%
\def\eg{\emph{e.g}\onedot} \def\Eg{\emph{E.g}\onedot}
\def\ie{\emph{i.e}\onedot} \def\Ie{\emph{I.e}\onedot}
\def\cf{\emph{c.f}\onedot} \def\Cf{\emph{C.f}\onedot}
\def\etc{\emph{etc}\onedot} \def\vs{\emph{vs}\onedot}
\def\wrt{w.r.t\onedot} \def\dof{d.o.f\onedot}
\def\etal{\emph{et al}.}
\def\st{\emph{s.t}\onedot}
\makeatother

\usepackage{xspace}
\newcommand{\name}[0]{FAGC\xspace}
\usepackage{color,xcolor}
\newcommand{\HK}[1]{\textcolor{red}{[KunHe: #1]}}
\newcommand{\BLUE}[1]{\textcolor{blue}{#1}}
\newcommand{\red}[1]{\textit{\textcolor{red}{#1}}}

\newcommand{\real}{\mathbb{R}}
\newcommand{\bt}{\Theta}
\newcommand{\hbt}{\hat{\Theta}}

%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> Figure/robustness_original.tex <==
\begin{figure*}[tb]
    \centering
    \includegraphics[width=0.9\textwidth]{Fig/robustness.pdf}
    \vspace{-10pt}
    \caption{Comparison of classification error of models on rotated and sheared images}
    \vspace{-10pt}
    \label{fig:robustness}
\end{figure*}

==> Table/int_sc.tex <==
\begin{table}[tb]
\centering
\caption{Test error ($\%$) of the baselines with square kernels (\textit{Square}) and the corresponding modified versions with circular kernels (\textit{Circle}) or integrated kernels (\textit{Int-SC}) on CIFAR-10 and CIFAR-100. 
%\textit{Square} and \textit{Circle} respectively indicate the existing CNNs with square kernels and the counterpart CNNs with circular kernels. \textit{Int-SC} indicates the integration of square and circular kernels. 
We run the model $5$ times for each dataset \& model setting to reduce the variance}
\small
\begin{threeparttable}[b]
%\resizebox{0.48\textwidth}{!}{
\begin{tabular}{lccc}
\toprule
\textbf{Model}&\textbf{Kernel}&\textbf{CIFAR-10}&\textbf{CIFAR-100}\\
%\cmidrule(lr){2-3}\cmidrule(lr){4-5} 
%&WRNCifar&DenseNetCifar&WRNCifar&DenseNetCifar\\
\midrule  
WRNCifar&{Square}      &$  4.33\pm0.10 $&$ 20.59\pm0.16  $ \\
WRNCifar&{Circle}      &$  4.44\pm0.12 $&$ 20.89\pm0.22  $ \\
WRNCifar&{Int-SC}      &$  4.20\pm0.11 $&$ 20.48\pm0.12  $ \\ 
\midrule  
DenseNetCifar&{Square}      &$  5.26\pm0.11 $&$ 23.07\pm0.22  $ \\
DenseNetCifar&{Circle}      &$  5.32\pm0.09 $&$ 23.04\pm0.18  $ \\
DenseNetCifar&{Int-SC}      &$  5.06\pm0.04 $&$ 22.91\pm0.16  $ \\ 
\bottomrule
\end{tabular}
%}
\end{threeparttable}
%\vspace{-5pt}

\label{table:int_sc}
% \vspace{-5pt}
% \vskip -0.1in
\end{table}




% \begin{table*}[tb]
% \centering
% \begin{threeparttable}[b]
% \resizebox{0.8\textwidth}{!}{
% \begin{tabular}{lcccc}
% \toprule
% \multirow{2}{*}{\textbf{Model}}&\multicolumn{2}{c}{\textbf{CIFAR-10}}&\multicolumn{2}{c}{\textbf{CIFAR-100}}\\
% \cmidrule(lr){2-3}\cmidrule(lr){4-5} 
% &WRNCifar&DenseNetCifar&WRNCifar&DenseNetCifar\\
% \midrule  
% {Square}      &$  4.20\pm0.07 $&$ 4.25\pm0.10  $ &$ 20.59\pm0.18 $&$ 21.08\pm0.32 $\\
% {Circle}      &$  4.58\pm0.11 $&$ 4.39\pm0.17  $ &$ 21.25\pm0.14 $&$ 21.17\pm0.12 $\\
% {Int-SC}      &$  5.17\pm0.13 $&$ 4.86\pm0.09  $ &$ 22.45\pm0.15 $&$ 21.89\pm0.18 $\\ 
% \bottomrule
% \end{tabular}
% }
% \end{threeparttable}
% \vspace{-5pt}
% \caption{Test error ($\%$) of the baselines with square kernels (Square) and the corresponding circular kernel (Circle) versions in kernel size $k \in \{3,5,7 \}$ on CIFAR-10 and CIFAR-100. We run the model $5$ times for each dataset \& model setting to reduce the variance. With the increment of kernel size, the advantage of circular kernel over square kernel becomes more distinct.}
% \label{int_sc}
% %\vskip -0.1in
% \end{table*}









==> Table/large-circular-kernel.tex <==
\begin{table*}[htbp]
\centering
\caption{Test error ($\%$) of the baselines with square kernels (Square) and the corresponding circular kernel (Circle) versions in kernel size $k \in \{3,5,7 \}$ on CIFAR-10 and CIFAR-100. For a fair comparison, we use the original data without data augmentation. We run the model $5$ times for each dataset \& model setting to reduce the variance}
\begin{threeparttable}[b]
\resizebox{0.85\textwidth}{!}{
\begin{tabular}{lccrccr}
\toprule
\multirow{2}{*}{\textbf{Model}}&\multicolumn{3}{c}{\textbf{CIFAR-10}}&\multicolumn{3}{c}{\textbf{CIFAR-100}}\\
\cmidrule(lr){2-4}\cmidrule(lr){5-7} 
&Square&Circle&Test Err.$\downarrow$&Square&Circle&Test Err.$\downarrow$\\
\midrule

VGG ($3 \times 3$) &$  10.75
\pm0.10 $&$ 10.40\pm0.31 $&$\textbf{\BLUE{0.35}}$ 
&$ 36.39\pm0.15 $&$ 34.74\pm0.09 $&$\textbf{\BLUE{1.65}}$\\

VGG ($5 \times 5$) &$ 11.27\pm0.22 $&$ 9.79\pm0.23 $&$\textbf{\BLUE{1.48}}$ 
&$ 37.92\pm0.43 $&$ 34.61\pm0.20 $&$\textbf{\BLUE{3.31}}$\\

VGG ($7 \times 7$) &$  12.78\pm0.11 $&$ 11.24\pm0.32  $&$\textbf{\BLUE{1.54}}$ 
&$ 40.97\pm0.24 $&$ 37.46\pm0.16 $&$\textbf{\BLUE{3.51}}$\\ 
\midrule

ResNet ($3 \times 3$)&$  11.22\pm0.16 $&$ 10.72\pm0.21 $&$\textbf{\BLUE{0.50}}$ 
&$ 42.45\pm0.43 $&$ 40.03\pm0.35 $&$\textbf{\BLUE{2.42}}$\\
ResNet ($5 \times 5$)&$  12.97\pm0.25 $&$ 11.42\pm0.13 $&$\textbf{\BLUE{1.55}}$ 
&$ 43.67\pm0.53 $&$ 41.28\pm0.19 $&$\textbf{\BLUE{2.39}}$\\
ResNet ($7 \times 7$)&$  14.51\pm0.35 $&$ 12.27\pm0.47 $&$\textbf{\BLUE{2.24}}$
&$ 46.89\pm0.11 $&$ 41.53\pm0.67 $&$\textbf{\BLUE{5.36}}$\\
\midrule

WRNCifar ($3 \times 3$)  
&$  14.13\pm0.06 $&$ 11.70\pm0.52  $&$\textbf{\BLUE{2.43}}$ 
&$ 33.34\pm0.48 $&$ 32.99\pm0.57 $&$\textbf{\BLUE{0.35}}$\\
WRNCifar ($5 \times 5$)     
&$ 12.92\pm0.40 $&$ 10.39\pm0.39  $&$\textbf{\BLUE{2.53}}$ 
&$ 36.51\pm0.13 $&$ 34.38\pm0.10 $&$\textbf{\BLUE{2.13}}$\\
WRNCifar ($7 \times 7$) 
&$  10.70\pm0.08 $&$ 8.73\pm0.22  $&$\textbf{\BLUE{1.97}}$ 
&$ 39.97\pm0.33 $&$ 36.81\pm0.64 $&$\textbf{\BLUE{3.16}}$\\ 
\midrule
DenseNetCifar ($3 \times 3$)
&$  8.41\pm0.08 $&$ 8.30\pm0.42 $&$\textbf{\BLUE{0.11}}$ 
&$ 30.83\pm0.28 $&$ 29.72\pm0.50 $&$\textbf{\BLUE{1.11}}$\\
DenseNetCifar ($5 \times 5$)
&$  8.59\pm0.18 $&$ 7.94\pm0.07 $&$\textbf{\BLUE{0.65}}$ 
&$ 30.84\pm0.10 $&$ 29.26\pm0.20 $&$\textbf{\BLUE{1.58}}$\\
DenseNetCifar ($7 \times 7$)
&$  8.92\pm0.06 $&$ 7.93\pm0.01 $&$\textbf{\BLUE{0.99}}$
&$ 32.53\pm0.62 $&$ 29.81\pm0.32 $&$\textbf{\BLUE{2.72}}$\\
\bottomrule
\end{tabular}
}
\end{threeparttable}
% \vspace{-5pt}
% With the increment of kernel size, the advantage of circular kernel over square kernel becomes more distinct.}
\label{large-circular-kernel}
%\vskip -0.1in
\end{table*}


